A Closer Look at Small-loss Bounds for Bandits with Graph Feedback

We study small-loss bounds for adversarial multi-armed bandits with graph feedback, that is, adaptive regret bounds that depend on the loss of the best arm or related quantities, instead of the total number of rounds. We derive the first small-loss bound for general strongly observable graphs, resolving an open problem of Lykouris et al. (2018). Specifically, we develop an algorithm with regret $\mathcal{\tilde{O}}(\sqrt{\kappa L_*})$ where $\kappa$ is the clique partition number and $L_*$ is the loss of the best arm, and for the special case of self-aware graphs where every arm has a self-loop, we improve the regret to $\mathcal{\tilde{O}}(\min\{\sqrt{\alpha T}, \sqrt{\kappa L_*}\})$ where $\alpha \leq \kappa$ is the independence number. Our results significantly improve and extend those by Lykouris et al. (2018) who only consider self-aware undirected graphs. Furthermore, we also take the first attempt at deriving small-loss bounds for weakly observable graphs. We first prove that no typical small-loss bounds are achievable in this case, and then propose algorithms with alternative small-loss bounds in terms of the loss of some specific subset of arms. A surprising side result is that $\mathcal{\tilde{O}}(\sqrt{T})$ regret is achievable even for weakly observable graphs as long as the best arm has a self-loop. Our algorithms are based on the Online Mirror Descent framework but require a suite of novel techniques that might be of independent interest. Moreover, all our algorithms can be made parameter-free without the knowledge of the environment.

==> LowerBound.tex <==
\subsection{Lower Bound}\label{lower bound}

We begin with the negative result that shows the impossibility of achieving small-loss bound for general weakly observable graphs. The proof is done by contradiction. The idea is that if such algorithm exists, then we can design an adversary that forces this algorithm to overfocus on one weakly observable node $u$ and seldom choose the node $v$ that can observe it. Then the adversary can make $u$ bad without letting the algorithm notice that, which will make the algorithm miss an even better node and thus not achieve small-loss bound. Formally, we have the following theorem.
\begin{theorem}
    For any weakly observable graph, there exists an adversary such that, no algorithm can achieve $\tilde{\mathcal{O}}\left(L^\star\right)$ regret, where $L^\star$ is the loss of the best node in hindsight.
\end{theorem}
\begin{proof}
     Since the graph is weakly observable, there must exist two nodes $u,v$, such that $u$ doesn't have a self-loop and $v$ can't observe $u$. Suppose there exists an algorithm $\mathcal{A}$ that achieves $\tilde{\mathcal{O}}(L^\star)$ regret. Then consider the following adversary: $\ell_{t,u}=0,~\ell_{t,v}=T^{-\frac{1}{2}}$, and $\ell_{t,w}=1, \forall w\ne u,v$. We call nodes other than $u,v$ ``bad arms''. Note that the loss of each node is constant over time and $L^\star=0$. Because $\mathcal{A}$ achieves $\tilde{\mathcal{O}}(L^\star)$ regret, bad arms must be played at most $o(T^{\epsilon_1})$ times in expectation for any $\epsilon_1>0$ and $v$ can be played at most ${\mathcal{O}}( T^{\frac{1}{2}+\epsilon_2})$ times in expectation for any $\epsilon_2>0$. The former condition means we can find a time interval of length ${{\Omega}}(T^{1-\epsilon_1})$ such that $\mathcal{A}$ plays bad arms less than $\frac{1}{2}$ time in expectation in this time interval. Therefore, by Markov Inequality, we have with probability $\frac{1}{2}$, $\mathcal{A}$ doesn't play bad arms at all in this time interval. Now we switch the loss of $u$ to $1$ in this time interval. Notice that with probability $\frac{1}{2}$ $\mathcal{A}$ can't notice the change because $u$'s loss is not revealed to the algorithm when it chooses $u$ or $v$. Since $v$ must be played ${\mathcal{O}}( T^{\frac{1}{2}+\epsilon_2})$ times in total, we conclude that the algorithm plays $u$ at least $\Omega(T^{1-\epsilon_1})$ in this time interval and therefore suffers ${{\Omega}}(T^{1-\epsilon_1})$ regret. This makes a contradiction because in this adversary, $v$ is the best arm and $L^\star=L_v=T^{\frac{1}{2}}$.
\end{proof}
The construction is inspired by Theorem 6 in \citep{DBLP:journals/corr/abs-1905-12950}. Despite the negative result for true small-loss bound for any weakly observable graph, we can still prove some adaptive regret bound for it. We start from considering a special group of weakly observable graphs.
